Rabia: Simplifying State-Machine Replication Through Randomization

We introduce Rabia, a simple and high performance framework for implementing state-machine replication (SMR) within a datacenter. The main innovation of Rabia is in using randomization to simplify the design. Rabia provides the following two features: (i) It does not need any fail-over protocol and supports trivial auxiliary protocols like log compaction, snapshotting, and reconfiguration, components that are often considered the most challenging when developing SMR systems; and (ii) It provides high performance, up to 1.5x higher throughput than the closest competitor (i.e., EPaxos) in a favorable setup (same availability zone with three replicas) and is comparable with a larger number of replicas or when deployed in multiple availability zones.

==> 4f+1.tex <==
% \begin{figure*}[t]
% \begin{minipage}{.48\textwidth}
%   \centering
%   \includegraphics[width=\textwidth]{img/Rabia-eval-fast-path-line.pdf}
%   \caption{Throughput vs. Median Latency plots. \name{} is configured with an optimized fast path ($n = 5$ and $f = 1$). Both systems have client batch size $= 10$, and \name{} has proxy batch size $= 10$. %Both systems have up to $300$ clients. 
%   \lewis{@Roger: run Rabia client = 400 and add the final two points on the plot.}}
%   %\caption{Rabia: $5-1$ setup, proxy batch size = 20. The number of closed-loop clients goes from 20 to 300, while Epaxos' number of clients goes from 20 to 500.  client batch = 10}
%   \label{fig:5-1-close}
% \end{minipage}
% \hfill
% \begin{minipage}{.48\textwidth}
%   \centering
%   \includegraphics[width=\textwidth]{img/Rabia-eval-fast-path-bar.pdf}
%   \caption{Throughput with different number of replicas. \name{} is configured with an optimized fast path $(n=4f+1)$. Both systems do not use client batching, and \name{} has proxy bath size $=100$. \lewis{@Roger: fix number in parenthesis. Remove n=3.}}
%   %\caption{Rabia: $5-1$ setup, proxy batch size = 100. 4-CPU machines, 500 closed-loop clients for Epaxos, and Rabia. 50 percent write. No client batching.}
%   \label{fig:5-1-scalability}
% \end{minipage}
% \end{figure*}

\begin{figure*}[t]
\begin{subfigure}{.48\textwidth}
\centering
\includegraphics[width=\linewidth]{img/Rabia-eval-zone-cb1.pdf}
\caption{Client batch size $= 1$.}
%\caption{Availability Zone Test, proxy batch is fixed to 20. Dots at each line correspond to 20, 40, 60, 100, 160, 260, 360, and 460 clients, respectively. This graphs shows two lines that have client batch size = 1 for your reference. The number in the parentheses means client batch size}
%\label{fig:diff}
\end{subfigure}
\begin{subfigure}{.48\textwidth}
\centering
\includegraphics[width=\linewidth]{img/Rabia-eval-zone-cb10.pdf}
\caption{Client batch size $= 10$.}
%\caption{Availability Zone Test, proxy batch is fixed to 20. Dots at each line correspond to 20, 40, 60, 100, 160, 260, 360, and 460 clients, respectively. This graph shows all four lines. The number in the parentheses means client batch size}
\end{subfigure}
\caption{Throughput vs. 99-th percentile Latency plots. \name{} is deployed in a 3-replica system with proxy batch size $=20$. ``\name - diff'' denotes the case when each replica is deployed in a distinct availability zone in GCP. \name{} has a moderate decrease in throughput across multiple availability zones. The performance loss is smaller with the increased throughput. There is no obvious increase in 99-th percentile latency.}
\label{fig:diff-whole}
\end{figure*}

==> SMR.tex <==
\section{Preliminary}
\label{s:preliminary}

\lewis{I need to rewrite this part.}

We consider an asynchronous system consisting of $n$ nodes with unique IDs $\{1, \dots, n\}$. Up to $f$ nodes may crash in the system. We do not consider Byzantine faults. We assume that the set of nodes is static. Efficient reconfiguration of our system is left as an interesting future work. 

\subsection{Randomized Binary Consensus}

One way to circumvent the FLP impossibility \cite{FLP} is to relax the termination property. Ben-Or proposed the following formulation of the binary consensus problem \cite{Ben-Or_PODC83}:

\begin{itemize}
    \item \textit{(Randomized) Termination}: Each non-faulty node generates an output with probability $1$. In other words, as time proceeds, the probability for a node to dice on an output value approaches to $1$.
    \item \textit{Agreement}: Each non-faulty node generates the same output.
    \item \textit{Validity}: The output must be some node's input.
\end{itemize}

The key to Ben-Or's algorithm is using a randomization trick -- picking $0$ or $1$ with equal probability (random coin flip) -- to break tie. Ben-Or's algorithm takes exponential rounds in expectation. \lewis{define round?}

After Ben-Or's seminal work, a few papers made randomized consensus algorithms more piratically, including  a multi-valued version, i.e., the input space is more than three \cite{Raynal_ISORC01,Chen_IPL09}, and the usage of shared coin.

\subsection{A Simple Solution to Multi-Decree Consensus}

Aforementioned algorithms only solved single-decree consensus, whereas typical applications (e.g., SMR) require multi-decree consensus. A simple solution is to us a multi-valued randomized consensus to agree on a command for each slot. 


Performance issue.

==> alg.tex <==
\section{Binary BC Algorithm}

\newcommand{\maj}{\textsc{Maj}}
\newcommand{\majv}{\textsc{MajV}}

\begin{itemize}
    \item Binary consensus.
    
    \item Basically Ben-Or + Common-Coin
    
    \item Each phase has two rounds, round 1 and round 2.
    
    \item $R[p, t]$ is a \textit{multi-set} of received values in round $t$ at phase $p$.
    
    %\item $\#(b, R)$ is the number of occurrence of $b$ in a multi-set $R$.
    \item $\maj(R) = $ the number of occurrence of the majority non-$?$ value in a multi-set $R$.
    
    \item $\majv(R) = $ the majority non-$?$ value in a multi-set $R$.
    
    \item Line \ref{line:CommonCoinFlip} makes sure that every node flips the coin same number of times.
\end{itemize}


\begin{algorithm*}[!hptb]
\begin{algorithmic}[1]
	\small
	
	\item[{\bf Local Variables}: /* These variables can be accessed and modified by any thread at $i$. */]{}
    \item[] $x$ \COMMENT{input at node $i$, $\{0, 1\}$}
    \item[] $v[t,1]$ \COMMENT{a vector of local state at round $1$, $\{0, 1\}$}
    \item[] $v[t,2]$ \COMMENT{a vector of local state at round $2$, $\{0, 1, ?\}$} 
    
    \item[] $p$ \COMMENT{phase, integer}
    
    \item[] \hrulefill

\begin{multicols}{2}

    \item[{\bf When Binary Consensus is invoked:}]
    \STATE $v[0, 1] \gets x$
    \STATE $p\gets 0$
    \WHILE{$TRUE$}
        \item[\hspace{25pt}/* Round 1 */]
        \STATE Send ($i, p, 1, v[p, 1]$) to all 
        \STATE \textbf{wait until} $|R[p, 1]| \geq n-f$
        %\IF{$\exists b$~s.t.~$\#(b, R[p, 1]) \geq \lfloor\frac{n}{2}\rfloor+f+1$}
        \IF{$\maj(R[p, 1]) \geq \lfloor\frac{n}{2}\rfloor+f+1$}
            \STATE Send $(i, \majv(R[p, 1]), DEC)$ to all
            \STATE \textbf{Output} \majv(R[p, 1])
        %\IF{$\exists v$~s.t.~$|\{v \in R[r, 1]\}| > \frac{n}{2}$}
        %\ELSIF{$\exists b$~s.t.~$\#(b, R[p, 1])\geq \lfloor\frac{n}{2}\rfloor + 1$}
        \ELSIF{$\maj(R[p, 1])\geq \lfloor\frac{n}{2}\rfloor + 1$}
            \STATE $v[p, 2] \gets \majv(R[p,1])$
        \ELSE
            \STATE $v[p, 2] \gets ?$
        \ENDIF
        
        ~
        
        \item[\hspace{25pt}/* Round 2 */]
        \STATE Send ($i, p, 2, v[p, 2]$) to all
        \STATE $randBit \gets \textsc{CommonCoinFlip}()$\label{line:CommonCoinFlip}
        \STATE \textbf{wait until} $|R[p, 2]| \geq n-f$
        \IF{$\maj(R[p, 2]) \geq f+1$}\label{line:majv>=f+1}
            \STATE Send $(i, \majv(R[p,2]), DEC)$ to all
            \STATE \textbf{Output} $\majv(R[p,2])$
        \ELSIF{$\maj(R[p, 2])\geq 1$}
            \STATE $v[p+1,1] \gets \majv(R[p, 2])$ \label{line:maj-value}
        \ELSE
            \STATE $v[p+1, 1] \gets randBit$ \label{line:coin-value}
        \ENDIF
        \STATE $p \gets p+1$ \COMMENT{Proceed to next phase}
    \ENDWHILE
    
    \item[]

    \item[/* Event handler: executing in background */]
    %\item[/* Event handler: executing atomically in]
    %\item[background, even after node $i$ decides */]

    \item[{\bf Upon receiving $(j, p, t, b)$ from node $j$}:]
    \STATE Add $b$ to $R[p,t]$
    
    \item[{\bf Upon receiving $(j, b, DEC)$ from node $j$}:]
    \STATE \textbf{Output} $b$

\end{multicols}
\end{algorithmic}
\caption{BO-BC: Code for node $i$}
\label{algo:RandCon}
\end{algorithm*}


\subsection{Correctness}

Validity is obvious.

\begin{lemma}
\label{lemma:same-value-1}
For any $p \geq 1$, if all nodes reaching phase $p$ with $v[p,1] = v$, then all nonfaulty nodes decide on $v$ no later than phase $p$.
\end{lemma}

This is because $\majv(\cdot) = v$.

\begin{lemma}
\label{lemma:some-node-decide}
For any $p \geq 1$, if some node decides on $v$ in phase $p$, then all nonfaulty nodes either decide on $v$ in phase $p$ or set $v[p+1,1] = v$. 
\end{lemma}

This is because line \ref{line:majv>=f+1} of BO-BC.

Lemma \ref{lemma:some-node-decide} implies agreement.

\begin{lemma}
\label{lemma:termination-probability}
For any phase $p \geq 2$, the probability that all nonfaulty nodes decide by phase $p$ is at least $1/2$.
\end{lemma}

\begin{proof}
Consider two cases:

\begin{itemize}
    \item \textit{Case I}: all nonfaulty nodes set $v[p, 1] = randBit$, the result of the common coin, in phase $p-1$ (each node executes line \ref{line:coin-value}). 
    
    By assumption of the common coin and Lemma \ref{lemma:same-value-1}, all nodes decide on $randBit$ in phase $p$.
    
    \item \textit{Case II}: some node sets $v[p, 1] = \majv(\cdot) = v$ (executing line \ref{line:maj-value}) in phase $p-1$. 
    
    Each node has only three choices in phase $p-1$ (i) decides on $v$ in phase $p-1$, (ii) executes line \ref{line:maj-value}, and (iii) executes line \ref{line:coin-value}. 
    
    Choice (i) is impossible; Choice (ii) can only set $v[p,1] = v$ by a simple quorum intersection argument.
    
    In case (iii), the return value of the common coin of phase $p$ is $v$ for all nodes with probability $1/2$. Thus, by Lemma \ref{lemma:same-value-1}, all nonfaulty nodes decide on $v$ in phase $p$.
\end{itemize}
\end{proof}

\begin{theorem}
\label{thm:expected-constant-time}
BO-BC has expected round complexity $4$.
\end{theorem}

\begin{proof}
By Lemma \ref{lemma:termination-probability}, the probability of terminating after one phase is at least $1/2$. Therefore, the probability of terminating after $t$ phases is at least

\[
(1-\frac{1}{2})^{t-1} \frac{1}{2}
\]

This implies that the number of phases until termination is upper bounded a geometric random variable whose expected value is $1/2$. Therefore, the expected number of phase is $2$.

Since each phase has two rounds, the expected number of round is $2*2 = 4$.
\end{proof}

\section{Original Ben-Or}

\begin{algorithm}[!hptb]
\begin{algorithmic}[1]
	\small
	\STATE $state \gets x_i$ \COMMENT{$x_i$ is the input}
	\STATE $p \gets 1$ \COMMENT{Start with Phase 1}
    \WHILE{$true$}
        \STATE /* Round 1 */
        \STATE Send ($\state, p, state$) to all 
        \STATE \textbf{wait until} receiving $\geq n-f$ phase-$p$ \state~messages
        \IF{value $v$ appears $\geq \lfloor\frac{n}{2}\rfloor + 1$ times }
            \STATE $vote \gets v$
        \ELSE
            \STATE $vote \gets ?$
        \ENDIF
        \STATE /* Round 2 */
        \STATE Send ($\vote, p, vote$) to all
        \STATE \textbf{wait until} receiving $\geq n-f$ phase-$p$ \vote~ messages
        \IF{value $v$ appears $\geq f+1$ times}
            \STATE \textbf{Output} $v$
        \ELSIF{value $v$ appears at least once}
            \STATE $state \gets v$
        \ELSE
            \STATE $state \gets \textsc{CoinFlip}()$ \COMMENT{coin flip}
        \ENDIF
        \STATE $p \gets p+1$ \COMMENT{Proceed to next phase}
    \ENDWHILE
\end{algorithmic}
\caption{Ben Or's Algorithm}
\label{algo:ben-or}
\end{algorithm}

==> proof.tex <==
\section{Safety Proof}
\label{app:safety-proof}

\section{Liveness Proof}

\subsection{Proof of Lemma \ref{lemma:termination-probability}}
\label{app:lemma-proof}

\begin{proof}
Consider two cases:

\begin{itemize}
    \item \textit{Case I}: all replicas that have not crashed yet set $state = \textsc{CommonCoinFlip(p-1)}$ in phase $p-1$ (each replica executes line 26). 
    
    By the assumption of the common coin, these replicas decide on $\textsc{CommonCoinFlip(p-1)}$ in phase $p$.
    
    \item \textit{Case II}: some replica sets $state = v$ (executing line 24) in phase $p-1$. 
    
    There are only three possible scenarios for each non-faulty replica in round $2$ of phase $p$: (i) execute \textsc{FindReturnValue}$(v')$ at line 22, (ii) execute $state \gets v'$ at line 24, and (iii) execute $state \gets \textsc{CommonCoinFlip}(p-1)$ at line 26. 
    
    By a simple intersection argument and how the round 1 is devised, we can see that $v'$ must equal to $v$ in scenario (i) and (ii).
    Now consider scenario (iii). Since the common coin returns $0$ and $1$ by an equal chance, $\textsc{CommonCoinFlip}(p-1)$ returns $v$ with probability $1/2$. In other words, all replicas that have not crashed yet will start with phase $p$ with the same value $v$ with probability at least $1/2$.
    Thus, all the non-faulty replicas will execute \textsc{FindReturnValue}$(v)$ in phase $p$ with probability $\geq 1/2$. This completes the proof.
\end{itemize}
\end{proof}

==> prooflisting.tex <==

\lstdefinelanguage{ivy}{
  keywordstyle=[1]{\ttfamily\color{keywordcolor}},
  showstringspaces=false,
  keepspaces=true,
  basicstyle=\ttfamily\footnotesize,
  columns=[l]fullflexible,
  belowskip=-0.2 \baselineskip,
  %% numbers=left,
  %% numberstyle=\small, 
  %% numbersep=8pt,
}

\subsection{Ivy Proof}
\lstinputlisting[language=ivy]{weak_mvc.ivy}

\vspace{3em}
\subsection{Coq Proof}
\lstinputlisting[language=ivy]{weak_mvc.v}

==> redis-performance.tex <==
\begin{figure}[t]
\begin{subfigure}{.42\textwidth}
  \centering
  \includegraphics[width=\textwidth]{sosp-img/redis-thpt-noBatching.pdf}
  \caption{Batching}
  \label{fig-sub:redis-nobatching}
\end{subfigure}
\begin{subfigure}{.42\textwidth}
  \centering
  
  \includegraphics[width=\textwidth]{sosp-img/redis-thpt-batching.pdf}
  \caption{No Batching}
  \label{fig-sub:redis-batching}
\end{subfigure}%


\caption{Throughput. The deployment consists of 3 4-CPU replica machines with co-located clients. Both systems have client batch size $=10$.}
\label{fig:redis}
\end{figure}


==> related.tex <==
\section{Related Work}

\subsection{System Work}

\begin{itemize}
    \item Mencius: \url{ https://www.usenix.org/legacy/events/osdi08/tech/full_papers/mao/mao.pdf}
    
    \item EPaxos: \url{https://www.cs.cmu.edu/~dga/papers/epaxos-sosp2013.pdf}
    
    \item CAESAR: \url{https://arxiv.org/pdf/1704.03319.pdf}
    
    \item Leaderless State-Machine Replication: Specification, Properties, Limits
    
    \item State-machine replication for planet-scale systems

    (The later two are by Pierre, and can be found here \url{https://sites.google.com/site/0track/publications?authuser=0})
    
    \item Maybe some Proof-of-Stake protocols?
\end{itemize}




\subsection{Theory Work}

\begin{itemize}
    \item Ben-Or PODC83 \cite{Ben-Or_PODC83}: \url{https://dl.acm.org/doi/10.1145/800221.806707}
    
    This version might be easier to read: \url{https://arxiv.org/pdf/cs/0209014.pdf}
    
    \item Ittai Abraham DISC10 \cite{Abraham_DISC10}: \url{https://www.microsoft.com/en-us/research/publication/fast-asynchronous-consensus-with-optimal-resilience/}
    
    \item Michel Raynal ISORC01 \cite{Raynal_ISORC01}: \url{https://ieeexplore.ieee.org/document/922837/}
    
    \item Michel Raynal SRDS04 \cite{Raynal_SRDS04}: \url{https://ieeexplore.ieee.org/document/1353024/}
    
    \item Wei Chen \cite{Chen_IPL09}: \url{https://www.sciencedirect.com/science/article/abs/pii/S0020019009001884?via\%3Dihub}
\end{itemize}






